A Machine Learning Approach for Smartphone-based Sensing of Roads and Driving Style

Road transportation is of critical importance for a nation, having profound effects in the economy, the health and life style of its people. With the growth of cities and populations come bigger demands for mobility and safety, creating new problems and magnifying those of the past. New tools are needed to face the challenge, to keep roads in good conditions, their users safe, and minimize the impact on the environment. This dissertation is concerned with road quality assessment and aggressive driving, two important problems in road transportation, approached in the context of Intelligent Transportation Systems by using Machine Learning techniques to analyze acceleration time series acquired with smartphone-based opportunistic sensing to automatically detect, classify, and characterize events of interest. Two aspects of road quality assessment are addressed: the detection and the characterization of road anomalies. For the first, the most widely cited works in the literature are compared and proposals capable of equal or better performance are presented, removing the reliance on threshold values and reducing the computational cost and dimensionality of previous proposals. For the second, new approaches for the estimation of pothole depth and the functional condition of speed reducers are showed. The new problem of pothole depth ranking is introduced, using a learning-to-rank approach to sort acceleration signals by the depth of the potholes that they reflect. The classification of aggressive driving maneuvers is done with automatic feature extraction, finding characteristically shaped subsequences in the signals as more effective discriminants than conventional descriptors calculated over time windows. Finally, all the previously mentioned tasks are combined to produce a robust road transport evaluation platform.

==> template/aprobacion.tex <==
\newgeometry{
    top=3cm, 
    bottom=1cm, 
    left=4.5cm, 
    right=3cm
}

\newpage
\thispagestyle{empty}

\noindent
\justify
\vTitulo. Disertación presentada por \vAutor como requisito parcial para obtener el grado de \vGrado, ha sido aprobada y aceptada por:

\vspace*{-1.8cm}
\hspace*{-3.5cm}
\includegraphics[keepaspectratio=true,height=2.5cm]{template/uach.png}
\vspace*{1cm}

\noindent\line(1,0){250} \\
\textbf{M.I. Javier González Cantú} \\
Director de la Facultad de Ingeniería \\

\vspace*{8mm}

\noindent\line(1,0){250} \\
\textbf{Dr. Alejandro Villalobos Aragón} \\
Secretario de Investigación y Posgrado \\

\vspace*{6mm}

\noindent\line(1,0){250} \\
\textbf{Dr. Alejandro Villalobos Aragón} \\
Coordinador Académico \\

\vspace*{6mm}

\noindent\line(1,0){250} \\
\textbf{\vDirectorTesis} \\
Director de Tesis \\

\vspace*{6mm}

\noindent
\textbf{\vFecha} \\

\vspace*{6mm}

\noindent
Comité: \\

\vComite

\vspace*{2cm}

\hspace*{8cm}\fbox{
    \begin{minipage}{16em}
    \centering
    \textcopyright \hspace{1ex} Derechos Reservados\\
    \textbf{\vAutor}\\
    Circuito Universitario Campus II,\\
    Chihuahua, Chih., México.\\
    \vFecha
    \end{minipage}
}

\restoregeometry    

==> template/portada.tex <==
\newgeometry{
    top=2.5cm, 
    bottom=1cm, 
    left=2cm, 
    right=2cm
}

\thispagestyle{empty}

\begin{center}

    \LARGE{ \textbf{ \textsc{
        Universidad Autónoma de Chihuahua
    } } }    
    
    \vspace*{3mm}
    \Large{ \textbf{ \textsc{
        Facultad de Ingeniería
    } } }    
    
    \vspace*{4mm}
    \large{ \textbf{ \textsc{
        Secretaría de Investigación y Posgrado
    } } }  
    
    \vspace*{5mm}
    \line(1,0){300}
    
    \vspace*{1.5cm}
    \includegraphics[keepaspectratio=true,]{template/uach.png}
    
    \vspace*{1cm}
    \huge{ \textbf{ \textsc{
        \vTitulo
    } } }    
    
    \vspace*{1cm}
    \normalsize{ 
        \textsc{
            por:
        } 
    }  
    
    \vspace*{5mm}
    \LARGE{ \textbf{ \textsc{
        \vAutor
    } } }   
    
    \vspace*{7mm}
    \normalsize{
        \textsc{
            disertación presentada como requisito para obtener el grado de 
        } 
    }
    
    \vspace*{5mm}
    \Large{ \textbf{ \textsc{
        \vGrado
    } } }   
    
\end{center}

\vspace*{5cm}
\normalsize{ 
    \textsc{
        Chihuahua, Chih., México.
        \hspace*{9cm}
        \vFecha
    }
}

\restoregeometry    


